Distribution free optimality intervals for clustering

We address the problem of validating the ouput of clustering algorithms. Given data $\mathcal{D}$ and a partition $\mathcal{C}$ of these data into $K$ clusters, when can we say that the clusters obtained are correct or meaningful for the data? This paper introduces a paradigm in which a clustering $\mathcal{C}$ is considered meaningful if it is good with respect to a loss function such as the K-means distortion, and stable, i.e. the only good clustering up to small perturbations. Furthermore, we present a generic method to obtain post-inference guarantees of near-optimality and stability for a clustering $\mathcal{C}$. The method can be instantiated for a variety of clustering criteria (also called loss functions) for which convex relaxations exist. Obtaining the guarantees amounts to solving a convex optimization problem. We demonstrate the practical relevance of this method by obtaining guarantees for the K-means and the Normalized Cut clustering criteria on realistic data sets. We also prove that asymptotic instability implies finite sample instability w.h.p., allowing inferences about the population clusterability from a sample. The guarantees do not depend on any distributional assumptions, but they depend on the data set $\mathcal{D}$ admitting a stable clustering.

==> sdp-kmeans-computation.tex <==
 % section removed completely from JRSS
\subsection{Computational considerations}
Our experiments have shown that, currently, with the generic SDP solver SDPNAL$++$ \cite{}, very good guarantees for K-means clusterings can be obtained for data sets in the thousands. 

The worst-case complexity the SDP algorithms being $O(n^6)$ \cite{}, we cannot hope that direct solving can handle very large data sets. However, the SS problems such as \ref{eq:mebound} have many features that can be exploited to accelerate the computation. First, the current solution $X(\clust)$ is a good starting point. Second, since the number of constraints is large, column generation techniques could be very promising. One could heuristically to detect the data points that most constrain the solution. These are the points that lie near the cluster boundaries. These points would be the ones for which subproblems would be solved i... The removal of the ``easy points'' in the aspirin experiments is a simple application of such a technique. \mmp{put the points back and check solution}

A third approach is to divide-and-conquer. If the data is well-separated into just two subsets of clusters, then one could solve two SS problems on the subsets. From the partial solutions  sometimes a global solution with an optimality certificate can be constructed, and otherwise a very good initial point can be obtained.

Besides, we observed consistently that the BTR does not vary with the sample size $n$. This suggests that in the future stochastic approaches (e.g. subsampling the data) could be proved to offer similar guarantees with the deterministic ones we obtained. 


==> sdp-kmeans-jrss20-resilience.tex <==
% OMITTTED from -jmlr18 journal paper. To be included in a future paper.
\section{Stability versus resilience}
\label{sec:resil}
The term clustering \emph{resilience}, introduced by
\citep{biluLinial:09}, represents an alternate definition of data
\emph{clusterability}. For a recent treatment of the matter, we refer
the readers to \cite{makarychev:}. Resilience applies to clusterings
in metric spaces. Hence, within this section, we redefine the data set
$\dataset$ to represent the set of distances between all pairs of data
points, i.e. $\dataset_{ij}=||x_i-x_j||$, and understand that
$\loss(\dataset,\clust)$ is a function of the cluster labels and the
distances. A dataset $\dataset'$ is an $\alpha$-dilation of
$\dataset$, $\alpha>0$, iff for each pair $i,j$ with $i,j\in[n]$,
$\dataset_{ij}\leq \dataset'_{ij}\leq (1+\alpha)\dataset_{ij}$. A
clustering $\clust$ is $(\alpha,\epsilon)$ \emph{resilient} iff
$\clust$ is the optimal clustering for $\loss(\dataset,\clust)$ and,
for any $\dataset$ $\alpha$-dilation of $\dataset$,
$\clust'=\operatorname{argmin}_{\clustal}\loss(\dataset',\clust')$ is
at distance $\distance$ no more than $\epsi$ from $\clust$.

It has been shown that if a data set has an $(\alpha,\epsilon)$
resilient clustering for $\alpha$ sufficiently large, then a nearly
optimal clustering can be found efficiently
\cite{awasthiCKS:15,awasthiBlumSheffet:12,awasthiBV:icml14,awasthiBlumSheffet:12,awasthiBlumSheffet:10},
\cite{biluLinial:09}, \cite{coleFR:15},
\cite{balcanL:16,balcanHW:16,balcanLG:14}. \cite{ben-david:arxiv15}
offers a critical survey of this area, and underscores that the
clusterability conditions are in general  restrictive, that is, $\alpha\geq 1+\sqrt{2}$.

Other papers \cite{} guarantee efficient recovery of a nearly optimal
clustering under a stability condition similar to ours. The optimal
clustering $\clust\opt$ of a data set is called
$(\delta,\epsi)$-\myemph{stable} \citep{} iff any clustering with
$\loss(\dataset,\clust)\leq \loss(\dataset,\clust\opt)+\delta$ is no
more than $\epsi$ in $\distance$ from $\clust\opt$.

Note that none of these papers discusses how to verify the assumptions
of $(\alpha,\epsilon)$-resilience or $(\delta,\epsi)$-stability. Here
we show that by the SS method one can obtain a certificate of
$(\delta,\epsi)$-stability or of resilience.

\begin{prop}\label{prop:stab2} Let $\loss$ be a clustering loss function that has a convex relaxation over $\X$, and let $X^*$ be the solution of the relaxed clustering problem \eqref{} for a given data set $\dataset$.  Let $\delta$ denote the solution of the following SS problem,
  \beq
\probe\quad \delta\,=\,\min_\X<X^*,X'>\quad \text{s.t. }\loss(\dataset,X')\leq \loss^*+\alpha
  \eeq
  for some $\alpha>0$.
  Then, for any  $\clust,\clust'$ clusterings satisfying
%\beq
$
\loss(\dataset,\clust),\,\loss(\dataset,\clust)\leq \loss^*+\alpha,
$
%\eeq
we have (1)
%\beq
$||X(\clust)-X(\clust')||^2_F\leq  8(K-\delta)$,
%\eeq
and, (2), $\distance(\clust,\clust')\leq \epsi=8(K-\delta)\pmax$ whenever $\epsi\leq \pmin$.
\end{prop}
%
%Stability also implies resilience, but the converse is not true for useful values of the resilience parameter $\alpha$. 
\begin{prop}\label{prop:stab-resil}
Let \loss~be Lipschitz w.r.t. the data, i.e. $|\loss(\dataset, X)-\loss(\dataset',X)|\leq \lambda ||\dataset-\dataset'||$ for all $X\in \X$. Denote by $\alpha_s$ the supremum over all $a>0$ so that the SS problem with level $\loss\opt+a$ results in $\epsilon\leq\pmin$. Then, if $2\alpha\lambda||\dataset||_F\leq \alpha_s$, the optimal clustering $\clust\opt$ is $(\alpha, 2\alpha\lambda||\dataset||_F)$ resilient. 
\end{prop}
The theorem above applies to the K-means loss. Note that $\lossk$ is Lipschitz in $D$, the squared distance matrix, rather than $\dataset$. In this case, resilience is obtained by replacing $\alpha$ with  $\sqrt{1+\alpha}-1$ in Proposition \ref{prop:stab-resil}. Hence, the SS method provides a tractable way to prove an otherwise intractable property. 

